Understanding Older Adults' Perceptions and Challenges in Using AI-enabled Everyday Technologies

Artificial intelligence (AI)-enabled everyday technologies could help address age-related challenges like physical impairments and cognitive decline. While recent research studied older adults' experiences with specific AI-enabled products (e.g., conversational agents and assistive robots), it remains unknown how older adults perceive and experience current AI-enabled everyday technologies in general, which could impact their adoption of future AI-enabled products. We conducted a survey study (N=41) and semi-structured interviews (N=15) with older adults to understand their experiences and perceptions of AI. We found that older adults were enthusiastic about learning and using AI-enabled products, but they lacked learning avenues. Additionally, they worried when AI-enabled products outwitted their expectations, intruded on their privacy, or impacted their decision-making skills. Therefore, they held mixed views towards AI-enabled products such as AI, an aid, or an adversary. We conclude with design recommendations that make older adults feel inclusive, secure, and in control of their interactions with AI-enabled products.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> contents/oldversion_discussion.tex <==
\subsection{Older Adults' Perceptions of AI}
Our survey study showed that older adults rated their knowledge level of AI as low, which is also in line with previous research~\cite{Bristows:survey}. However, despite our participants' limited knowledge of AI, they could \textit{recognize the use of AI} in most of the products listed in our survey. Their recognition of using AI in the products is attributed to their \textbf{perceived smartness} even though they found that AI used in only about 30\% of the products was  smarter than a human (See Sec.~\ref{subsec:OA's Knowledge}). 
% They further mentioned that AI would always have limitations despite fine-tuning it. 
Moreover, the perceived smartness also impacted their attitude and motivation to use a product. A previous study by Shin and Lee~\cite{shin2014effects} discussed the product's perceived smartness played a critical role in influencing a customer's understanding of the product's advantages and user acceptance. Our study found that an AI-enabled product's perceived smartness not only helped older adults identify its benefits but also its disadvantages. 
Our participants' perceptions of smartness of AI were two-fold: i) \textit{AI as assistance}, and ii) \textit{AI as a nuisance or a threat}. They shared various instances explaining how AI helped them in their day-to-day activities; at the same time, they also reported their concerns about AI as a threat to their privacy and a tool to accomplish vicious agendas. 

Prior research~\cite{hautea2017youth,long2020ai,touretzky2019envisioning} indicated that to achieve AI literacy, a user should have an understanding that their data is used in AI-enabled products. We found that the awareness of the use of data in AI-enabled products was fairly low among our participants, as discussed in Sec.~\ref{subsec:OA's Knowledge}. Moreover, our participants reported that they were comfortable sharing their data with only less than a quarter (23\%) of the listed AI-enabled products in the survey. However, low awareness of the use of data in AI-enabled products and discomfort to share data seem to be consistent across all age groups~\cite{Bristows:survey} and not a unique phenomenon among older adults.


\subsection{Older Adults' Experiences and Challenges in Using AI}
Prior research~\cite{lee2015perspective,wang2011older,xie2007information} suggested that older adults' motivation to accept a product depends on product's perceived usefulness, ease of use, recommendation from close ones, and assistance in using a product. Additional to past work~\cite{lee2015perspective,wang2011older,xie2007information} we also found that older adults' introduction to latest AI-enabled products is dependent on knowledge gained about the usefulness of the product from friends/family, availability of the product in the market, consumer reports, and public opinions about the products expressed in reviews on online shopping websites. 

Similar to the findings of previous studies~\cite{champley2008preliminary,meyer1997age,tsai2012older}, our participants also found that the printed manuals were perceived easier to follow than online manuals. However, our participants reported that these days not every product (trending technology) provided a precise and articulately written printed manuals. Moreover, navigating an online user manual is another difficulty for them, and sometimes they did not even get the desired information. Similar to the list of design guidelines for creating senior-friendly instructions proposed by Fan and Truong that were mostly based on non-AI products ~\cite{fan2018guidelines}, future work should explore how these guidelines might need to be adapted to create effective and easy-to-use instructions, both printed and online, to assist older adults with using AI-enabled products. 

Furthermore, our participants found the results of voice-assistants and recommendation features on video platforms like YouTube and shopping sites like Amazon inefficient, frustrating, and counter-intuitive. The recommendation feature on shopping sites falsely advertised and communicated that the products that our participants were interested in are in stock; in a few instances, such recommendation features inundated an older adult's video platform with the repetitive content/genre, which they found annoying, as it limited their opportunity to engage with new content. Despite the problem of stale and unwanted recommendations were reported by prior studies like~\cite{fields2011analysis,wilhelm2018practical}, such issues still exist. 
Our participants adopted strategies to overcome the inaccuracies of AI-enabled voice assistants. Corresponding to a past work~\cite{druga2017hey} where children interacted and adopted strategies to extract answers from the voice-assistants, our participants added keywords such as adding 'quiet' to 'tell me a quiet bed-time story' to their commands while interacting with voice-assistants to get more accurate results when they were looked for subjective information than a factual answer like date or weather. 
% Additionally, Bigham and Carrington~\cite{}claimed that advancing AI technologies have started to disregard the needs of people with disabilities, like smart devices integrated with voice recognition technology abandon people who difficulty hearing or speaking.
% To evade the flood of same content by recommendation features on video platforms, our participants watched a video in incognito mode on the browser.

Our participants further shared that one of the key barriers in embracing AI is the lack of awareness of AI-enabled products and their usefulness among older adults. Consistent with the findings of recent literature~\cite{cave2018portrayals,chuan2019framing,ouchchy2020ai}, negative news about AI also made our participants reluctant to trust and use AI-enabled products; moreover, they felt AI technology is precipitously advancing, which made it hard for them to get acquaint with it constantly~\cite{vaportzis2017older}. 

The difference in technology adoption and confidence between gender groups was documented in past studies~\cite{goswami2015gender,yau2012gender}. Our study found that females were disinclined towards learning about the inner-functionalities of the AI-enabled products but were excited about using them, and females with partners depended on their partner to set-up AI-enabled products. However, due to the limited data samples, our study does not provide a generalized understanding of whether and how gender might play a role in the adoption of AI-enabled products among older adults and calls for further research investigation.   

Past work~\cite{ostrom2019customer} demonstrated factors like threats of data privacy, trusting AI-enabled products with unexplainable outcomes to make key decisions make users anxious in using an AI-enabled products, which also holds true for our participants. What's more, our participants felt some AI products, such as AI customer-service, were designed to make people feel being served by a real person but were not instrumental. Such feeling about AI could have negatively affect older adults' trust and use in AI-enabled products.
%help when they were stuck,  do not help an individual when they are stuck, which is crucial for an older adult to trusting and using a product~\cite{xie2007information}.
% Additionally, participants also struggled to understand the unexpected outcomes of AI-enabled products when they were anticipating for something else or wanted reasoning from the products behind their decisions and outcomes.

\subsection{Design Considerations}
In the findings section, we presented different expectations of older adults from the AI-enabled products~\ref{subsec:expectations}. Based on participants' experiences and expectations of using AI-enabled products, we discuss the design considerations to improve perceived usefulness and experiences of AI-enabled products for older adults in light of the past work.

\textbf{Make AI-enabled Products Affordable and Accompanied with Senior-Friendly Learning Resources}. Our participants desired \textit{affordable} AI-enabled products to cater to their aging needs. To cater to older adults' aging needs and minimize cognitive load, AI-enabled products should incorporate gradual disclosure and explanation of features~\cite{druga2017hey,long2020ai}. They mentioned conveying a product's usefulness and providing useful, well-structured \textit{senior friendly} learning materials like printed manuals over digital sources is crucial for adopting and using an AI-enabled product to its full potential~\cite{champley2008preliminary,meyer1997age,tsai2012older}.

\textbf{Help Older Adults Handle Privacy and Security Concerns}. One of the main concerns and barriers in using AI-enabled products for older adults is the threat to their data privacy. Moreover, our participants find maintaining their privacy settings in an AI-enabled product complex. Therefore, they need the products to provide walkthroughs and reminders of privacy settings to inform and educate them about it. Golbeck and Mauriello~\cite{golbeck2016user} argued that a better presentation of privacy information could help users make informed decisions about which applications are safe to interact with and recommended using human-centered approaches to understanding the users and their behaviors to better deliver security information. Recently, Nora and Mentis~\cite{Nora2021BuildingforWe} showed that pairing older adults up to deal with privacy and security information together could be another viable approach. 


\textbf{Provide Explanations When AI-enabled Products' Behavior Deviates from Older Adults' Expectations}. We discovered that older adults feel puzzled when the outcomes of AI-enabled products do not match their expectations. Consequently, our participants expect explanations from the AI-enabled products in such situations. These clarifications also reinstate older adult's trust in AI-enabled products. Kocielnik et al.~\cite{kocielnik2019will} show that setting right expectations and shaping them with respect to an AI-enabled product improves product understanding and, thus, improves user acceptance of AI-enabled products. Further, to manage user’s expectations AI guidelines have been proposed to underscore the role of explaining AI-product behavior~\cite{amershi2019guidelines, abdul2018trends}. However, none of the studies have focused on older demographics. Consequently, we argue that it is important for our community to explore what explanations are expected from older adults for AI-enabled products when their behaviors deviate from older adults' expectations and how such explanations should be formatted and delivered to them.
% consider this one to inform a design recommendation
% \subsubsection{Match User's Expectations}
% For an older adult to fully embrace AI the outcome of the products must match users' expectations or it should effectively answer that they were looking for. For instance, participants shared that the voice-assistants defy users' commands and outwits them such as referring internet pages when asked about defining a term, narrating a noisy bedtime story when the user wanted to listen a calming bedtime story. Moreover, users notice differences in the way they are acknowledged by voice-assistants.  For instance, P7, thinks that the voice-assistants interact with her husband more dearly than her maybe because he used his voice-profile to set it up.
% \begin{quote}
%     P7: ``... She doesn't like to talk to me anyway, she talks to him because he's put his voice, his name, and everything in there, so she talks with him. I don't have all of that (Alexa's response) in there...well at night you know um he'll reset the alarm. For example, you know after that's done he'll say thank you, and she'll respond to him um you're welcome bob, or you betcha, or have a good night.''
% \end{quote}

% consider this one to inform a design recommendation
% \subsubsection{Be Self-Explanatory and Easy to Use}
% The AI-enabled product should be easy to use and should not require a user to hone any technological skills to use it. Our participants shared a common feeling that the technology today is designed for people who have enough background knowledge and awareness about data and AI. If a older adult lacks awareness about data privacy they can be taken deceived. So people suggested the products should be designed in a way that lets a user learn about maintaining their privacy.
% \begin{quote}
%     P15: ``... If it were easier to do the privacy settings... you have to know where to find your location in privacy settings. So I suppose, if there were um uh of an app that came up on your computer, or your iPhone, or your phone uh that was about privacy... I think the most helpful thing might be if there was a routine part just like the calendar or messages or whatever that can tell  where you're and where you can get a hold of your privacy settings and then walk you through them (privacy settings).'' 
% \end{quote}


\textbf{Make Older Adults Feel In Control When Using AI-enabled Products}. A few recent studies~\cite{amershi2019guidelines, abdul2018trends} outlined design guidelines, mostly based on younger populations, for AI-enabled products like providing controls to the user to manage the behavior of the product, notifying users about customization and updates. Similarly, our current work shows that older adults also expected AI-enabled products to provide them with options to control the decision-making process and the information that they want to consume rather than being  enforced to receive like advertisements.  However, it is worth noting that being able to control the settings of AI-enabled products well often demands some understanding or mental model of the underlying AI. In a few instances, our participants were reluctant to learn the underpinnings of a product and wanted the product to invisibly operate without them worrying about the inner-functionalities. Therefore, they wanted an alternative to learning or skipping the underpinnings of an AI-enabled product, which involved understanding if a product uses their data and how. This raises an open challenge for HCI and accessibility designer and researchers that how best to make older adults feel in control while also not requiring them to understand too much about the underpinning mechanism when using AI-enabled products. 
% providing an option to the older adults to know if a product uses their data and how is another critical design consideration builds their trust in the AI-enabled products.

% consider this one to inform a design recommendation
% \subsubsection{Offer Controls and Be Transparent}
% One of the barriers that older adults encountered in using AI-enabled products is to understand why the product did not respond the way it should. Moreover, they feel since AI is a trending technology the older adults not have an upper-hand to comprehend the outcomes. Therefore, they want the products to explain the reasoning behind their decision, which can gain their trusts on AI-enabled products. Moreover, they want control over the repeated advertisements they are shown whenever they search something. P12, suggested a dedicated platform that enable older adults to seek guidance in using and choosing a feature or an AI product.  
% \begin{quote}
%   P12: ``... I would like AI to give me options. I wish, I could filter, but I don't like that it just spits the information at you without giving you options... It would be nice to have a platform that you could go and say I have a question, and I can hard type my problems, and it would narrow down and take me to the solution gradually. For example, if I'm looking for a book, then, it should ask what kind of genre do you find interesting, oh I like this, okay, what have you read in the past... I would like if there's actually an independent and dedicated platform for asking questions...'' 
% \end{quote}
% Another desired aspect for AI-enabled products is the option to enable/disable transparency of the inner-workings of a product based on people's interest/knowledge level. This was suggested by P10 to relieve the older adults with limited knowledge of AI as transparency could be intimidating and hinder their opportunity to interact with the product. For instance,
% \begin{quote}
%     P10: ``... Invisibility, it's that they should just function in the background without you having to know that you're dealing with AI... because I think that would relieve suspicions of people who are frightened of it (AI)...''
% \end{quote}

% consider this one to inform a design recommendation
% \subsubsection{Be Inclusive}
% Participants urged the need to consider the aging needs of their demographic when designing AI products. For instance, participant, P3 mentions, 
% \begin{quote}
%     P3:``... You know our sensory abilities decline with aids. So, definitely uh um uh the options to increase the size of print or audible cues versus reading cues. Maybe offering very simple baby step type tutorials uh online maybe putting them on YouTube or um you know in a CD that's uh you know... and um maybe even a uh um a helpline that uh you know that's a 1-800 line or a chat line where uh that is accessible and can be easily reached, where we can ask questions if we're stumped.''
% \end{quote}

% What's more, participants suggested that the AI-enabled products should be financially accessible to the older adults because most of them live on pensions. P4 suggests that the AI-enabled products should be affordable for older adults to use, which is as follows:
% \begin{quote}
%     P4: ``Definitely financial because what over 50 percent of seniors live on social security so it has to be financially approachable for a senior.''
% \end{quote}



==> contents/oldversion_findings.tex <==
% \subsection{General Perceptions of Older Adults about AI}
% \label{subsec:OA's General Perception}

% \subsubsection{Identifying the use of AI in different products}
% \subsection{Knowledge of AI}
% \subsubsection{AI vs. Human Intelligence}
% \subsubsection{AI --- Perceived good or bad?}
% \subsubsection{Data Literacy}
% \subsubsection{Sources to Learn AI}

% \subsubsection{Survey Results}
% We asked the respondents to report their AI knowledge level by choosing a score on a scale of 1 to 5, as shown in Table~\ref{tab:knowledgelevel}, most of the (57\%) older adults reported having some knowledge about AI. We then presented a list of AI learning sources as shown in Table~\ref{tab:learningsources} with an ``other'' option to the respondents to select or provide sources that they used to learn anything about AI. The most used learning source is ``Internet search'' followed by ``Friends/Family members'' and ``Newspaper''; apart from the listed source, older adults also reported other learning sources like radio and news channels.

% Our survey findings showed that respondents used a variety of AI-enabled products. 
% % 18\% of the $11$ listed AI-enabled products are always used, as presented in Figure~\ref{fig:experienceAI}. 
% The most frequently used AI-enabled products are search engines like Google, 27 out of 35 respondents use it, followed by navigational applications like Google Maps (25 out of 35) and email spam filter (16 out of 35) and online shopping recommendation feature (16 out of 35). However, respondents rarely used customer service chatbots (7 out of 35), recommendation systems on video platforms such as Netflix (11 out of 35), voice-assistants like Alexa (11 out of 35), and none of our respondents (0 out of 35) used Robotic Vacuums.

% We asked respondents whether they considered the AI-enabled products smart and if they thought AI-enabled products were smarter than humans. Respondents considered search engines like Google (20 out of 35) the smartest followed by navigational applications like Google Maps (16 out of 35) and voice-assistants like Alexa (13 out of 35). In contrast, when asked about products smarter than humans, a similar trend was observed. Search engines were selected by most of the respondents (14 out of 35) who felt this AI-enabled product was smarter than humans followed by navigational applications like Google Maps (11 out of 35) and voice-assistants like Alexa (6 out of 35).

% Our survey revealed that most of our survey respondents prefer using various types of AI products irrespective of their age and limited knowledge of AI. Moreover, respondents leverage search engines, newspapers, and depend on families and friends to learn about AI. However, we do not know yet the reasons for limited knowledge of older adults in AI technology and their sparse use of certain AI products.

% The survey study helped us in identifying the older adults who use AI-enabled products but, we still did not have a deep understanding of: i) the experiences of older adults in using AI-enabled products, ii) if they face any difficulties in using AI-enabled products (and what), iii) how their experiences with AI-enabled products inform their perception of AI technology, iv) their expectations from the AI technology. Therefore, to answer those questions and understand the experiences of older adults in detail, we conducted online semi-structured interviews.


% Next, we present key themes derived from interviews to further illustrate older adults' perceptions and understanding of AI. % In this section, we present the findings of older adults' \textit{perceptions and understanding of AI}, \textit{personal experiences}, and \textit{challenges in using AI-enabled products}, and \textit{ expectations for AI-enabled products}. Wherever appropriate, we first report quantitative insights from the survey and then provide qualitative findings from the interviews. 

% \subsection{Perceptions and Understanding of AI (RQ1)}

% \label{subsec:OA's Experience}
% Our survey brought forth a general perception of older adults about AI. We asked respondents to choose from a list of products (refer section for the list of products shown to respondents in the survey~\ref{subsubsec:materials}) that they thought use AI and found that they recognized the use of AI in about 64\% of the listed AI products, as shown in Figure~\ref{fig:recognizeAI}.
% We asked respondents whether they considered the AI-enabled products were smart and whether they thought AI-enabled products were smarter than humans. Figure~\ref{fig:smartAI} shows the result. Respondents considered that approximately 51\% of the AI-enabled products were smart. In contrast, only approximately 30\% of the products were considered to be smarter than humans.
% When asked to share their feelings about the use of AI in different products, in Figure~\ref{fig:concernAI} we see, around 39\% of the products that use AI concerned respondents; at the same time, the use of AI in 28\% of the products made them unsure about their feelings towards AI. To gauge respondents' data literacy, we posed questions about their awareness on the use of their data in the AI-enabled products, and if they were comfortable sharing their data with those products. We found that respondents were aware of 33\% of the AI-enabled products that use their data, but they were uncertain about using their data for the other 30\% of the products, Figure~\ref{fig:dataliteracy}. At the same time, they were only comfortable using their data for 23\% of the listed AI-enabled products, as shown in, Figure~\ref{fig:dataliteracy}. We asked the respondents to report their AI knowledge level by choosing a score on a scale of 1 to 5, as shown in Table~\ref{tab:knowledgelevel}, most of the (55\%) older adults report having some knowledge about AI. We then presented a list of AI learning sources as shown in Table~\ref{tab:learningsources} with an ``other'' option to the respondents to select or provide sources that they used to learn anything about AI. The most used learning source is ``Internet search'' followed by ``Friends/Family members'' and ``Newspaper''; apart from the listed source, older adults also reported other learning sources like radio and news channels.

% \begin{table}[]
% \caption{This table lists the AI learning sources that older adults use to learn about AI; the respondents specified radio and news channels as other learning sources. Participants were allowed to select multiple learning sources that they used to learn AI.} 

% \label{tab:learningsources}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lr}
% \toprule
% \textbf{{AI Learning Sources}}                             & \textbf{{No. of Survey Responses}} \\ \bottomrule
% Internet search (e.g., Google)                                          & 23 (18.40\%)                              \\
% Friends or family members                                               & 22 (17.60\%)                              \\
% Newspapers                                                                  & 22 (17.60\%)                          \\
% Online video sharing platforms (e.g., Youtube)                          & 11 (8.80\%)                               \\
% TV channels                                                             & 11 (8.80\%)                               \\
% Movies                                                                  & 10 (8.00\%)                                       \\
% Social media (e.g., Facebook, Twitter)                                  & 10 (8.00\%)                                       \\
% Others (please specify)                                                 & 8  (6.40\%)                                      \\
% Academic articles (e.g., computer science journal or conference papers) & 6  (4.80\%)                                      \\
% Massive open online course (e.g., Coursera, edX)                        & 2  (1.60\%)                                    \\
% \bottomrule
% \end{tabular}
% %
% }
% \end{table}



% \begin{table}[]
% \caption{This survey data shows the self-reported AI knowledge levels among older adults.} 
% \label{tab:knowledgelevel}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{clc}
% \toprule
% \textbf{Self-reported Score}  & \textbf{AI Knowledge Level}                                        & \textbf{No. of Survey Participants}\\
% \bottomrule
% 1 & I am not aware of anything about AI.                      & 0   (0.00\%)          \\
% 2 & I am aware of AI but do not have much knowledge about it. & 12  (34.28\%)             \\
% 3 & I have some knowledge about AI.                           & 20  (57.14\%)          \\
% 4 & I am knowledgeable about AI.                              & 3   (0.085\%)        \\
% 5 & I am very knowledgeable about AI.                         & 0   (0.00\%)       \\
% \bottomrule
% \end{tabular}
% %
% }
% \end{table}


% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\columnwidth]{FIG/recognizeAI.png}
%   \Description[Pie chart displaying the percentage of products that use AI recognized by respondents.]{The chart presents that respondents recognized the use of AI in 64\% of the $11$ listed products, and 36\% of them were not recognized. Respondents were allowed to select multiple products that they thought use AI.}
%   \caption{Pie chart of the recognized products that use AI by respondents.}
%   \label{fig:recognizeAI}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\columnwidth]{FIG/humanvs.png}
%   \Description[Pie charts displaying the percentage of products perceived smart on the left and smarter than humans by respondents on the right.]{On average, the left chart reports that 51\% of the $11$ listed AI-enabled products were opted as smart, for 36\% products considered not smart, and for rest 13\% products respondents were unsure; whereas, the right chart shows 30\% of the $11$ listed products were considered smarter than humans by respondents, 48\% not smarter than humans, and unsure for 22\% of products.}
%   \caption{Pie charts of the products that were perceived smart, demonstrated on the left, and were considered smarter than humans, by respondents is shown on the right.}
%   \label{fig:smartAI}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{FIG/data_literacy.png}
%   \Description[Pie charts displaying the percentage of products for which respondents were aware of the use of their data, displayed on the left and percentage of products for which respondents were comfortable sharing their data, shown on the right.]{The left chart demonstrates that for 33\% of the $11$ listed AI-enabled products, respondents were aware that the products use their data, for 37\% not aware, and for 30\% unsure. However, in the right chart, respondents reported that they feel comfortable sharing their data with 23\% of the $11$ listed AI-enabled products, not comfortable for 38\% , and unsure for 39\% of the products.}
%   \caption{Pie charts of the products for which respondents were aware about their data use in the them, shown on the left, and were comfortable sharing their data, displayed on the right.}
%   \label{fig:dataliteracy}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\linewidth]{FIG/concernAI.png}
%   \Description[Pie chart displaying the percentage of products that concern respondents about the use of AI in them.]{The chart shows that respondents were concerned about using AI in 39\% of the $11$ listed AI-enabled products, whereas for unsure how they feel for 28\% of the products.}
%   \caption{Pie chart of the products that concern respondents about the use of AI in them.}
%   \label{fig:concernAI}
% \end{figure}

\subsubsection{As an Aid to Save Efforts}
Participants perceived AI as an aid that helped them accomplish various day-to-day tasks with ease. Continuous advancements in technology such as improvements in voice recognition systems was beneficial in making a phone call or ordering a TV program to watch. Moreover, features like spelling suggestions on smartphones and keyword suggestions on Amazon shopping website minimized the participants' cognitive load while interacting with the product. Navigation applications like Google Maps, Waze made the world more accessible to them. Furthermore, AI-enabled products like Google Search, Alexa enabled them to access desired information instantly. Participants also found AI applications such as smart washer systems, switching on/off security cameras, and driving safety features in cars useful and convenient. 
\begin{quote}
    P14: ``... I like being able to see a print out of the message on my answering machine um I like the fact that I can make a phone call just using my voice, I can order up a television program.''
\end{quote}

\subsubsection{As a Spy to Direct Targeted Advertisements}
Most of the participants (P2, P3, P5, P8, P9, P10, P12) considered AI as a tool that tracks their online browsing behavior and collects data about them to direct targeted advertisements and steer their data search in a specific direction. They further shared that AI gathers information about their preferences --- their likes and dislikes --- through their computer and phone usage. The advertisements are catered towards the things they have either searched on a browser or have communicated to voice assistants. A few participants (P7, P14) also shared that their smartphone and voice-assistant eavesdrop on their conversation happening near them to advertise certain things from the conversation. For instance,
\begin{quote}
    P7: ``... If I have a conversation about something, and I'm not sure if this is what happens but I'll get ads on my Facebook page let's say for things that I've talked about uh with my husband or with friends or on the phone. So I know that she's (Alexa) listening, so that's uh that's the first thing that makes me aware of AI.''
\end{quote}
Participants found these experiences annoying and threatening. For example, P6, fears that personalized advertisement recommendations could enable someone to track and harm them. 
\begin{quote}
    P6: ``... I do get concerned when I'll look up something, I'll google something uh a pub a place to go visit, or uh a piece of you know a pair of pants, or something, and then I'll see all kinds of pop-ups about pants or Scotland, you know, I get concerned about that... what if I look for something to buy and then somebody decides oh we're gonna go get all the people who buy that thing and we're gonna do something to them.''
\end{quote}

% \subsubsection{A Learner to Increase its Specificity}
% \subsubsection*{\textbullet{}Learning from the past}
% A few participants acknowledge AI as a learning software that enhances its performance to make precise decisions based on the customer's data like current GPS data. Furthermore,it uses the data one inputs and their past online behavior to categorize their likes/dislikes and tendencies to predict their future behavior to make relevant recommendations. 
% \begin{quote}
%     P15: ``... I think it's used primarily through mathematics through algorithms and probability to get data and predict various things. So they use big data bases like a dictionary or maps or whatever and then they learn by the experience of the person who's using it. Where did they go, what do they want, what do they say, so you can add to it sometimes and the machine is supposedly learning that's what makes it intelligent, and it's used generally to predict things or to suggest things like spelling.''
% \end{quote}


% \subsubsection{As Pinocchio to Pretend to Te a Real Human}
\subsubsection{ AI Simulates Human Intelligence}
While a few participants (P2, P7, P12) drew parallels between the AI's intelligence and functioning to the human intelligence and brain to make decisions. They also pointed out AI's desperation to think and act as humans but no matter how many enhancements are made there are always going to be limitations. P7 compares Alexa to 'Pinocchio', a character from the story Pinocchio, who dreams of being a real boy. 
\begin{quote}
    P7: ``... I always think of the story of Pinocchio, well, he always wanted to be a real boy and I think that she wants to be a real girl but she's not a real girl and you just have to accept the fact that AI is going to always have limitations, they (AI) may get better but they may not be able to perfect it.''
\end{quote}
Participants also reported that they mistook a Chatbot for a actual human answering their questions until it asked for their feedback objectively (Yes/No) for every answer.

\subsubsection{As a Weapon to Fulfil Malicious Agenda}
Participants also perceived AI as tool to fulfil selfish maligning agendas of government, cyber attackers, and big tech companies. The interviewees worried that the government can have an upper hand over their data and can interfere in people's lives. People's personal judgements can be distorted by using AI for disinformation. Furthermore, almost all the interviewees feel AI can be used for wrong reasons like identity theft, scams, and system hacking.
\begin{quote}
    P2: ``... I think that certain uses of AI can be misdirected now. Things like, all this stuff with twitter and whatnot, I don't know to what degree, say for example, the Russians are using AI to figure out you know what people might be sensitive to, to make them doubt that we have good voting systems and you know planting doubt in your head by listening to what people are saying, and then sort of capitalizing on that so all this stuff in the wrong hands be used for doing underhanded things.''
\end{quote}


\subsection{Personal Experiences with AI-enabled Products (RQ2)}
% Our survey findings showed that respondents used a variety of AI-enabled products; 18\% of the $11$ listed AI-enabled products are always used, as presented in Figure~\ref{fig:experienceAI}. The most frequently used AI-enabled products are search engines like Google, 28 out of 31 respondents use it, followed by navigational applications like Google Maps (25 out of 31) and Email Spam Filter (18 out of 31). However, none of our respondents (0 out of 31) used Robotic Vacuums, respondents rarely used customer service chatbots (7 out of 31), recommendation systems on video platforms such as Netflix (11 out of 31) and shopping platforms like Amazon (16 out of 31) , and voice-assistants (11 out of 31) like Alexa. 

Next, we discuss the personal experiences based on interview participants' feedback about adopting and learning AI-enabled products and their unique insights into how such products changed their interaction behavior.

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\linewidth]{FIG/experienceAI.png}
%   \Description[Pie chart displaying the percentage of respondents' frequency of use for AI-enabled products.]{The survey data shows that 34\% of the $11$ listed AI-enabled products are never used by respondents, whereas 18\% of the products are always used.}
%   \caption{Pie chart of respondents' frequency of use for AI-enabled products.}
%   \label{fig:experienceAI}
% \end{figure}

% \subsubsection{Adopting AI-enabled Products}
% \subsubsection*{\textbullet{} Serendipitous Discovery}
% Participants adopted an AI-enabled product not because of their active choices but rather accidentally discovering those. For instance, they either received such products as gifts or bought the AI-enabled products because other conventional non-AI products were out of stock. 
% \begin{quote}
%     P9: ``... I have to have a grandson who works at Amazon and gave me Alexa.''
% \end{quote}
% \begin{quote}
%     P5: ``... I went to the store and that's the only ones they had in stock because of the pandemic so many appliances were not being built because they couldn't put people in factories close together to build them. So I would not have bought a fancy smart washer and dryer normally, but that was the only one that I could find and I needed a washer.''
% \end{quote}


%A similar experience was also shared by P13 who wanted to use a rotary phone but the fact that it is archaic in nature and she does not have an option she is compelled to use a smartphone.   

% \begin{enumerate}
%     \item[i.] Gifts: Most of the participants mention that the AI products that they are using are gifted by their children or grand-children. For instance, participants P9 mentioned that his grandson gifted him Alexa, whereas, P15 shared that Tesla was gifted by her children.
%     \begin{quote}
%         P9: ``... I have to have a grandson who works at Amazon and gave me Alexa.''
%     \end{quote} 
    
%     \item[ii.] Unintended Purchase: A participant retrospects that her purchase of a smart washer and dryer was because that was the only product available in the market, and she would not have bought it if she had an option. 
%     \begin{quote}
%       P5: ``... I went to the store and that's the only ones they had in stock because of the pandemic so many appliances were not being built because they couldn't put people in factories close together to build them. So I would not have bought a fancy smart washer and dryer normally but the only one that i could find and i needed a washer.''
%     \end{quote}
%     A similar experience is also shared by another participant, P13, who wants to use rotary phones but the fact that it is archaic in nature and she does not have an option she is compelled to use a smartphone. 
% \end{enumerate}

% \subsubsection*{\textbullet{} Informed Choices}
% Several interviewees also made informed decisions about their purchases. Major sources they gained knowledge about products were consumer reports or recommendations from friends and relatives.
%     \begin{quote}
%         P4: ``... Most of the information on my products I either get from consumer reports, or I will read uh evaluations on Amazon occasionally...So, for like the automatic vacuum the Roomba I think it is okay I have no interest in that at all okay, and I don't have animals so I don't have to worry.''
%     \end{quote}
%         \begin{quote}
%         P14: ``... I'm more likely to enlarge what I've been doing try a new thing if I've had seen somebody do it or somebody said hey did you ever try yes okay um so that makes me curious to use a particular product or at least try it yeah. and if I'm willing to buy a particular product I talk to my friends to who's got what um particularly the ones whom I respect.''
%     \end{quote}

% Additionally, witnessing a product's usefulness through some personal encounters was another motivation for adoption.     \begin{quote}
%         P4: ``... I was in my son's house and we were talking about Alexa in his kitchen. When he used the word Alexa, it (the device) picked up and said what can I do for you, and I thought that was very interesting. That was before I ordered mine.''
%     \end{quote}
    
% \begin{enumerate}
%     \item[i.] Reviews on Consumer Reports: Many participants read consumer report and trust the information to learn about different AI products, it's usefulness, and reviews. This also helps them to stay up-to-date with the trending AI-enabled products. A few also refer to the reviews for a product listed on Amazon before purchasing it. For instance, P4 says, 
%     \begin{quote}
%         P4: ``...Most of the information on my products I either get from consumer reports or I will read uh evaluations on Amazon ocassionally...So, for like the automatic vacuum the Roomba I think it is okay i have no interest in that at all okay, and i don't have animals so I don't have to worry.''
%     \end{quote}
    
%     \item[ii.] Word of mouth recommendations: A few participants also said that if a friend/relative suggests something they definitely feel curious and excited to try that product. For example, participant, P14 mentions,
%     \begin{quote}
%         P14: ``... I'm more likely to enlarge what I've been doing try a new thing if I've had seen somebody do it or somebody said hey did you ever try yes okay um so that makes me curious to use a particular product or at least try it yeah. and if I'm willing to buy a particular product I talk to my friends to who's got what um particularly the ones that I respect.''
%     \end{quote}
    
%     \item[iii.] Curiosity through Vicarious Experiences: Another set of participants bought the products because they witnessed a product's usefulness through their friends/relatives experiences. 
%     \begin{quote}
%         P4: ``...I was in my son's house and they have a an Alexa and we were talking about Alexa in his kitchen and it was in the next room and he used the word Alexa and it perked up and said what can I do for you, and I thought that was very interesting. That was before I ordered mine, and I ordered the small one um just because I thought it was fun.''
%     \end{quote}
%     On the other hand, a few decided not to purchase an AI-enabled after learning the negative experiences of their friends or relatives.
%     \begin{quote}
%         P5: ``...I do know people who have Alexa and they've told me that you have to be careful what you say because it will prompt a response if you say something you didn't actually mean to say and all of a sudden it's telling you the weather or whatever and it's just because it picked up on a word.''
%     \end{quote}

%     \end{enumerate}
% \subsubsection{Learning to Use AI-enabled products}
% Participants learned more information about their products by reading instruction manuals. They tended to prefer printed manuals over online manuals because it was easier to look back information on printed manuals. However, not every product has a printed manual any more. The situation further aggravates when the product was new and there were no other online sources like YouTube videos to refer to.
% \begin{quote}
%      P2: ``... I got an iPhone for example uh I thought I would be smart and got the latest possible model so about three years ago I got an iPhone 10 XS and I realized pretty quickly I made a mistake because that was so new there was not much information on the internet on how to do things and if I asked a specific question to get advice they would have it like for an iPhone 7 or an iPhone 8 but they wouldn't have it for an iPhone 10 XS.''
% \end{quote}

% Many times manuals are not indexed and condensed properly, which makes extracting a piece of information challenging and time-consuming. Moreover a few times, the manuals do not have the information that the interviewees are looking for. The participants also struggle in understanding the language of the manual. For instance, 
% \begin{quote}
%     P10: ``... I find manuals often don't have enough information...
%     %When a manual doesn't have enough information, generally online there are some discussion groups where people will be talking about the fact that is not there then you can get the information from discussion groups...So the computer that I'm using is a Dell which is manufactured in the United States yeah manufacturing the manual is very easy to understand okay but the the monitor is Samsung made in Korea and 
%     and sometimes it's clear that the manual wasn't written by someone whose native language is English, so it took some time to interpret it correctly.''
% \end{quote}

% \subsubsection{AI Changing Interaction Behavior}
% \subsubsection{Efforts to Refine Results}
% Several participants reported that they use voice-assistants for asking factual questions like weather or news. The AI-enabled voice-based systems break when asked for more subjective questions. In situations, when participants looked for a specific output, they tried to interact with the voice-based system by appending a keyword to the question to refine the results.
% \begin{quote}
%     P7: ``... I find that I have to add to the keywords. For example, so I may say to her (Alexa) 'tell me a bedtime story' or 'tell me a quiet bedtime story' so I have to add the word 'quiet' to it (Alexa) um she (Alexa) gave me choices and I chose and when I chose I think it was I thought it was quiet but it wasn't quiet and um you know that kind of thing where I need to add additional keywords so that there are maybe five or six key words before she and I reach an agreement on what I want. I might ask for slow jazz, you know, I might ask for jazz music and I would have to ask her for 'slow' jazz uh 'quiet' jazz 'gentle' jazz, whatever, I just keep adding keywords to it until she comes up with what I need.''
% \end{quote}
% Similarly, for telephone trees, participants say to avoid inputting the digits and to speak to a customer representative directly , they use 'operator'.
% \begin{quote}
%     P10: ``...  I say operator it sometimes connects me to an operator.''
% \end{quote}

% \subsubsection{Recommendation Bubble --- Feedback Loop}
% Participants found personalized recommendations based on a user's online behavior could enhance their entertainment and shopping experience. However, such recommendations create a negative user experiences by putting them in a bubble and hindering them from exploring other diverse content/product on the platform.
% % \subsubsection*{\textbullet{}Video Recommendations}
% For example, participants found video recommendations on YouTube and Netflix extremely restraining as it inundates their platforms with similar content or genre. 
% \begin{quote}
%     P12: ``... When I start looking at um videos it seems to be um sometimes too much and then sometimes too specific. I'll watch it, I'll tell you for instance, I'll watch an accident connection sequence in YouTube and then I see all these options over and they're just violent violent violent, and that wasn't the reason that I watched this (accident connection sequence video) because it (accident connection sequence video) had a purpose, it was there, but all of a sudden it (recommendations on YouTube) just starts bringing all the stuff here, and it's almost like a shotgun blasted.''
% \end{quote}
% To overcome this, participants search a video in an incognito mode on the browser to avoid the recommendation system from swamping the platform with the specific genre of video.

% \subsubsection*{\textbullet{}Shopping Recommendations}
% Similarly, for shopping platforms like Amazon, participants experienced that the recommendation system suggests the user about similar product but those are inaccurate. Other times, these recommendation systems did false advertisements of the product. For instance,
% \begin{quote}
%     P8: ``... If I was reading a book uh you know if I would you know if I read a book uh about the holocaust, or I bought a book I would get a flood of recommendations for books by the author. I didn't buy the book because of the author, I bought the book because of the topic.''
    % So when they're not useful to me, they're not useful because they're they don't really address to not refined enough to address what i was interested in...
    % I was recently looking for slip covers for outdoor cushions and I wanted floral slip covers and for three days amazon kept sending me messages in my email for slip covers that were not floral slip covers they were geometric they were solid colors they were striped it was not refined to what i specifically needed.''
% \end{quote}

% \subsubsection*{Different Passwords for Different Platforms}
% To master using any online platform safely, one must ensure using a strong password that qualifies all the platform's requirements. However, the interviewees face managing passwords as challenging to retain as it is taxing cognitively. Consequently, this experience inhibits participants from interacting with products and platforms that require a complex process of creating and maintaining the passwords.
% \begin{quote}
%     P15: ``...  I had a PayPal account because I bought something had to have PayPal but I really don't like it. Besides that just enhances the whole uh business of passwords and changing passwords and how complicated are your passwords and how do you remember the goddamn things...each one requires a specific kind of password and oh my goodness the techies say we've got to make them change every month. Well that really drives me blooming nuts.''
% \end{quote}

\subsection{Challenges when Using AI-enabled Products (RQ2)}
% We find that on average, 10.94\% of the survey respondents (average aggregated over $11$ listed products with a total of $274$ responses) face difficulties in using an AI-enabled product. A few respondents also answered the open-ended question to report the main challenges they faced in using AI-enabled products. A few hurdles shared were a steep learning curve for using AI-enabled products, counter-intuitiveness of products such as Facebook. For instance S26, says,
% \begin{quote}
%     S26: ``Do not understand instructions. NOT USER FRIENDLY. Things show up and I do not want them there. This is why I quit FB.''
% \end{quote}
% Moreover, if older adults seek assistance in using a product, it is difficult to get self-help instructions for a product through chatbot customer service; deviation of AI-enabled product outcome from the expected outcome, and inability to understand what AI-enabled products require as input to perform its task. To summarize the above issues, we report the following survey participants' S13 and S40 frustrations with the chatbots, voice-assistants, and social networks::
% \begin{quote}
%     S13: ``Voice-assistants - Don't know how to get the info I want; Recommendations - Recommendations aren't accurate; Social network - Social network doesn't explicate options clearly.''
% \end{quote}
% \begin{quote}
%     S40: ``Chat App takes you around in circles. I had one instance that after 3 hours of try this and that it dumped me! no offer for a human being. ...Voice assistants often misunderstand me. Social networking isn't as comprehensive about my friends group as when it started. Snapchat is a nightmare for me! But it's my granddaughter's preferred method of conversation!
% \end{quote}
In this section, we discuss the challenges that older adults encountered when using AI-enabled products and the reasons for these hurdles. Participants encountered various hurdles due to the lack of awareness of AI and its perceived usefulness to older adults. Moreover, when AI-enabled products functioned unexpectedly, it made them anxious about their privacy, and ultimately their trust in these products.

\subsubsection{Hard-To-Keep-Up Trend}
The majority of the interviewees feel AI is a growing trend, and it is hard to keep pace with the advancing and ever-changing and complex technology AI.
\begin{quote}
    P11: ``... The other thing is just how rapidly everything gets updated and you have to keep learning it, you know, and you get older, you don't want to learn stuff all the time. It's not that interesting, you want to be able to just use stuff, even like the car. I've got a new car I'd like to be able to drive it without all of this (smart features like conversational agents) stuff and you know it does not have to say, see you every time I get out of the car... It just is all annoying you know life is um more complicated than it used to be, it feels more complicated and more unsafe.'' 
\end{quote}
Moreover, we notice that different gender-groups respond to AI-enabled products differently
%, which we discuss next.
%\subsubsection*{\textbullet{}Varying Interest across Gender-groups}
Female participants (P13, P14, P15) who live with their partners seem reluctant in setting up the AI-enabled products. %For example,
\begin{quote}
    P13: ``... I don't know why I let my husband handle all the technical stuff, I don't wanna, I can't do it. He said we get a new computer, he sets it up, and I don't do anything.'' 
\end{quote}
One of the participants also mentioned that she and most of her female friends care less about the inner working of a product, and just wanted to know if it could be used easily.
\begin{quote}
    P8 \textit({A female interviewee}): ``... I think for my colleagues and I don't know if it's gender specific, but for me and the women that I have lunch with or socialize with it's a procedure-based thing. We really don't care how it works. I don't care about the underpinnings...what we care is how to access AI what buttons do I push...''
\end{quote}

\subsubsection{Lack of Awareness of AI}
Lack of awareness and knowledge of AI-enabled products put older adults at a disadvantage to use the product efficiently.
\begin{quote}
    P1: ``... In the communication world there are so many things we can do now and in many cases uh I know I'm not using my um iPhone nearly as effectively as my observation is that my children and certainly our grandchildren uh are taking much more advantage of it. So that type of education is I think important and helpful.''
\end{quote}
The participants pointed out two main reasons for their lacking awareness of AI. The first is if an individual does not have a  community such as a workplace or learning centers they miss the opportunity to learn and grow from people about advancing technologies like AI. For example,
\begin{quote}
    P8: ``... I think it's (reason for lacking awareness of AI) not so much age as it is uh what you're doing, if you're not with people using it, doing it, you're out of the loop. There should be some sense of community, like either through workplace, or maybe from uh like someplace, where you see people around you using certain technology and then you leverage that, and then you learn...''
\end{quote}
The second cause mentioned for low awareness of AI in older adults and their apprehensions is because of the negative portrayal of AI-enabled products by media. For instance, P10 says,
\begin{quote}
    P10: ``... There's a lot of suspicion of AI technology...Every time uh Elon Musk's cars kill somebody it makes headlines, but what doesn't make headlines is the number of accidents that are prevented by this technology, which I think is much greater number...'' 
\end{quote}
The participants felt the product advertisements fail to convey the usefulness of the products.

\subsubsection{Privacy Threat}
One of the biggest challenges that the older adults faced is the threat of keeping their data private and secure because they felt they are more vulnerable and can be taken advantage of. Constant personalized  recommendations for products and TV shows used information that they browsed or were asked for, which was an invasion of their privacy. They shared that being unaware of how and who manages the accumulated data make them anxious about using an AI-enabled product. P15, mentions how she turns off the location data every time she is done using a product.
\begin{quote}
    P15: ``... Well the big one is privacy I am a little super crazy about keeping my privacy. So as I said, I turn location off, I close apps as soon as I use them, I turn my computer off when I'm not using it to unplug it, you know, I have all kinds of antiviral and try everything on it, I have ad blockers I don't get ads. It drives my husband nuts he gets ads all the time, but um I really I don't want to be bothered. I don't want that kind of waste of my time, let alone I'm always afraid, well is this some um you know Serbian tracker uh trying to get in. So as I said, I keep lots of privacy blockers on my internet and on my computers, and so i really don't want suggestions from AI unless I ask.''
\end{quote}

\subsubsection{Over-reliance on AI}
% \subsubsection*{\textbullet()Pause reflect and invest}
The participants worried that the growing use of AI in products to enforce viewing of repeated information could replace their intuitive decision-making skills. For example, a few participants (P8, P10) also said that the use of AI to make critical decisions in medicine to do an intrusive procedure or not is agitating. Moreover, the enthusiasm to buy an AI product and trust it is so contagious that people have stopped paying attention to details and do not think through the consequences before depending on such products.
\begin{quote}
    P10: ``... I find the young people to be very reliant, and what I would consider to be over-reliant on technology. So yeah, I think the failure is to not look at this AI as a tool rather than as an end product... AI has learned to distinguish what looks abnormal on a mammogram better than a human eye can do, okay, but abnormal doesn't necessarily mean scary. So the identification of greater abnormality has led to more invasive procedures to do diagnostic procedures.''
\end{quote}

% \begin{quote}
%     P8: ``... The other day I saw a program about an all electric car and how wonderful this will be and we'll be rid of needing these gasoline engines and everyone will want an electric car, and then there was a group of engineers and their enthusiasm was almost contagious, you know, now, until I was listening I had no yen to have an electric car. I mean about them and I know that it probably is going to be better and blah blah but I didn't feel enthusiastic about it, that enthusiasm was contagious and so, I do worry that we might buy into AI in a very broad way stock and barrel without proper discrimination guard rails caution.''
% \end{quote}

\subsubsection{Deviating From Their Expected Behavior}
Our participants also reported that their expectations did not match the outcome of an AI-enabled product. People found it frustrating when the AI-enabled product tried to change certain things in a way that the user was not intending. For example, P14 found the voice-assistant in the smartphone annoying when it replaces unfamiliar words with something totally different that the user never intended to use. Moreover, P2 shared that the voice-assistant fails to respond when he is driving and looking for instant responses. The erratic nature of such products puzzles the participants as it does not provide any explanation for their decisions. For example, P12, shares an anecdotal story where he expected the product to justify their decision.
\begin{quote}
    P12: ``When I went to my dentist, Google Map took me down one way and back another way. I don't understand that. Now that I become familiar with the area, I just go back the same way as I came in. When it (Google Map) did that, I got disoriented...I would appreciate the re-routing if it tells me a reason for it, like there's a construction, or an accident.''
\end{quote}
%participant P9 was waiting for the alarm to go off but voice-assistant did not let that happen as the music was playing; whereas, 
\subsubsection{Pretending to Be Helpful}
Participants further talked about AI-enabled customer services in forms of automated telephone trees and chat bots sometimes pretend to be helpful and were intentionally used by companies to trick and prevent them from getting any help. 
\begin{quote}
    P2: ``... I think they intentionally keep it (assistance) difficult to find because they don't want to spend a lot of time with people to do that right.''
\end{quote}
Sometimes, it also became difficult for an individual to distinguish between the human and the bot interacting with them. These experiences discourage older adults from using and trusting such AI-enable customer services. To provide a clearer understanding about the challenge we report the experience of participant, P8, with the AI customer service.
\begin{quote}
    P8: ``... I wanted to know more about my gas bill, so I got on the website there's a chat thing. I thought that the way it (chat) worked was that there was somebody sitting at a laptop and then directly responded to what I typed. But that was not the case. So it was almost as bad as the telephone tree and so I try never to use them.''
\end{quote}

\subsection{Expectations for AI-enabled Products (RQ3)}
\label{subsec:expectations}
%\subsection{AI for Older Adults}
Participants felt that AI could assist them towards their aging needs such as mobility, cognitive functioning, and driving. Numerous participants (P2, P3, P5, P9, P10) want AI to be efficiently used in early self-diagnosing of diseases. 
\begin{quote}
    P2: ``... I think using it for diagnostic purposes, something which is more trustworthy, where it's like a monster database where all of the known medical problems are in there and if something comes up they can ask the right questions, and get some direction as to how to proceed to deal with that. It'd be nice if something like that were available.''
\end{quote}

Next, we present the expectations of participants for AI-enabled products.

\subsubsection{Be Inclusive}
Participants urged the need to consider the aging needs of their demographic when designing AI products. For instance, participant, P3 mentions, 
\begin{quote}
    P3:``... You know our sensory abilities decline with aids. So, definitely uh um uh the options to increase the size of print or audible cues versus reading cues. Maybe offering very simple baby step type tutorials uh online maybe putting them on YouTube or um you know in a CD that's uh you know... and um maybe even a uh um a helpline that uh you know that's a 1-800 line or a chat line where uh that is accessible and can be easily reached, where we can ask questions if we're stumped.''
\end{quote}

What's more, participants suggested that the AI-enabled products should be financially accessible to the older adults because most of them live on pensions. P4 suggests that the AI-enabled products should be affordable for older adults to use, which is as follows:
\begin{quote}
    P4: ``Definitely financial because what over 50 percent of seniors live on social security so it has to be financially approachable for a senior.''
\end{quote}

% \subsubsection{Human-friendly AI Customer Service}
% Almost all the interviewees shared their frustration about their experiences with the AI customer service. They prefer human assistance when they face any impediments in using a product. Moreover, they suggest using AI to identify the struggles of a user with the product --- telephone tree/chatbot, or the AI-enabled product --- to connect them directly to a customer representative rather than leaving them to figure it out on their own. One of the many similar ideas shared by participant is  as follows:
% \begin{quote}
%     P2: ``...It would be nice if you had the AI feature built into something and it detected that you were doing the same thing multiple times with no success once in a while I will get a flag that says, I see you're having a problem okay try such and such and that I mean there's some intelligence built in there where it's observing is that the user has got a problem they can't get out of it would be nice in designing products, the products would say I see you're having a problem here's a number to call to get some customer support.''
% \end{quote}

\subsubsection{Be Self-Explanatory and Easy to Use}
The AI-enabled product should be easy to use and should not require a user to hone any technological skills to use it. Our participants shared a common feeling that the technology today is designed for people who have enough background knowledge and awareness about data and AI. If a older adult lacks awareness about data privacy they can be taken deceived. So people suggested the products should be designed in a way that lets a user learn about maintaining their privacy.
\begin{quote}
    P15: ``... If it were easier to do the privacy settings... you have to know where to find your location in privacy settings. So I suppose, if there were um uh of an app that came up on your computer, or your iPhone, or your phone uh that was about privacy... I think the most helpful thing might be if there was a routine part just like the calendar or messages or whatever that can tell  where you're and where you can get a hold of your privacy settings and then walk you through them (privacy settings).'' 
\end{quote}

\subsubsection{Match User's Expectations}
For an older adult to fully embrace AI the outcome of the products must match users' expectations or it should effectively answer that they were looking for. For instance, participants shared that the voice-assistants defy users' commands and outwits them such as referring internet pages when asked about defining a term, narrating a noisy bedtime story when the user wanted to listen a calming bedtime story. Moreover, users notice differences in the way they are acknowledged by voice-assistants.  For instance, P7, thinks that the voice-assistants interact with her husband more dearly than her maybe because he used his voice-profile to set it up.
\begin{quote}
    P7: ``... She doesn't like to talk to me anyway, she talks to him because he's put his voice, his name, and everything in there, so she talks with him. I don't have all of that (Alexa's response) in there...well at night you know um he'll reset the alarm. For example, you know after that's done he'll say thank you, and she'll respond to him um you're welcome bob, or you betcha, or have a good night.''
\end{quote}

\subsubsection{Offer Controls and Be Transparent}
One of the barriers that older adults encountered in using AI-enabled products is to understand why the product did not respond the way it should. Moreover, they feel since AI is a trending technology the older adults not have an upper-hand to comprehend the outcomes. Therefore, they want the products to explain the reasoning behind their decision, which can gain their trusts on AI-enabled products. Moreover, they want control over the repeated advertisements they are shown whenever they search something. P12, suggested a dedicated platform that enable older adults to seek guidance in using and choosing a feature or an AI product.  
\begin{quote}
   P12: ``... I would like AI to give me options. I wish, I could filter, but I don't like that it just spits the information at you without giving you options... It would be nice to have a platform that you could go and say I have a question, and I can hard type my problems, and it would narrow down and take me to the solution gradually. For example, if I'm looking for a book, then, it should ask what kind of genre do you find interesting, oh I like this, okay, what have you read in the past... I would like if there's actually an independent and dedicated platform for asking questions...'' 
\end{quote}
Another desired aspect for AI-enabled products is the option to enable/disable transparency of the inner-workings of a product based on people's interest/knowledge level. This was suggested by P10 to relieve the older adults with limited knowledge of AI as transparency could be intimidating and hinder their opportunity to interact with the product. For instance,
\begin{quote}
    P10: ``... Invisibility, it's that they should just function in the background without you having to know that you're dealing with AI... because I think that would relieve suspicions of people who are frightened of it (AI)...''
\end{quote}

